Exploring Cross-Utterance Speech Contexts for Conformer-Transducer Speech Recognition Systems

This paper investigates four types of cross-utterance speech contexts modeling approaches for streaming and non-streaming Conformer-Transformer (C-T) ASR systems: i) input audio feature concatenation; ii) cross-utterance Encoder embedding concatenation; iii) cross-utterance Encoder embedding pooling projection; or iv) a novel chunk-based approach applied to C-T models for the first time. An efficient batch-training scheme is proposed for contextual C-Ts that uses spliced speech utterances within each minibatch to minimize the synchronization overhead while preserving the sequential order of cross-utterance speech contexts. Experiments are conducted on four benchmark speech datasets across three languages: the English GigaSpeech and Mandarin Wenetspeech corpora used in contextual C-T models pre-training; and the English DementiaBank Pitt and Cantonese JCCOCC MoCA elderly speech datasets used in domain fine-tuning. The best performing contextual C-T systems consistently outperform their respective baselines using no cross-utterance speech contexts in pre-training and fine-tuning stages with statistically significant average word error rate (WER) or character error rate (CER) reductions up to 0.9%, 1.1%, 0.51%, and 0.98% absolute (6.0%, 5.4%, 2.0%, and 3.4% relative) on the four tasks respectively. Their performance competitiveness against Wav2vec2.0-Conformer, XLSR-128, and Whisper models highlights the potential benefit of incorporating cross-utterance speech contexts into current speech foundation models.

==> IEEEtran/README <==

August 26, 2015


IEEEtran is a LaTeX class for authors of the Institute of Electrical and
Electronics Engineers (IEEE) transactions journals and conferences.
The latest version of the IEEEtran package can be found at CTAN:

http://www.ctan.org/pkg/ieeetran

as well as within IEEE's site:

http://www.ieee.org/

For latest news, helpful tips, answers to frequently asked questions,
beta releases and other support, visit the IEEEtran home page at my
website:

http://www.michaelshell.org/tex/ieeetran/

Version 1.8b has a number of significant changes over the v1.8a release.
For a full history of changes, please read the file changelog.txt.
The most notable changes in this release include:

 1) Added new comsoc mode for the IEEE Communications Society.
    This mode (at present) only invokes the use of the newtxmath math fonts.
 
 2) Revised IEEEeqnarray column specifications to work with active " 
    (or other punctuation catcode changes) as with babel under the
    german or ngerman language modes. 
    Thanks to Stefan M. Moser for reporting this problem.

 3) Added \indexspace and other index related macros as newer versions of
    article.cls now do. These macros are needed to avoid an error when
    using the glossaries package.
    Thanks to Sebastian Nyberg for suggesting this change.

 4) Fixed odd/even page header font bug under compsoc mode and
    other page style code improvements.
    Thanks to Marco Paolieri for reporting this problem.

 5) Added hooks to allow for easy control of spacing above title.

 6) Added the \IEEEnoauxwrite command.
    Thanks to Sudarshan Mukherjee for suggesting this feature.


NOTE: Take care not to confuse the "comsoc" and "compsoc" class
options/modes as they are very different:

comsoc  ==> IEEE Communications Society
compsoc ==> IEEE Computer Society

The comsoc mode requires that an acceptable Times math font be available on
the LaTeX system. This requirement will be enforced by IEEEtran in comsoc
mode. Either the freely available newtxmath font by Michael Sharpe
http://www.ctan.org/pkg/newtx
(version 1.451, July 28, 2015 or later is recommended)
or the commercial MathTime font (e.g., mtpro2.sty) is acceptable.
See Section II-D (2.4) "Class Options - comsoc, compsoc, transmag" of
the IEEEtran HOWTO for more details.


Best wishes for all your publication endeavors,

Michael Shell
http://www.michaelshell.org/


********************************** Files **********************************

README                 - This file.

IEEEtran.cls           - The IEEEtran LaTeX class file.

changelog.txt          - The revision history.

IEEEtran_HOWTO.pdf     - The IEEEtran LaTeX class user manual.

bare_conf.tex          - A bare bones starter file for IEEE conference papers.

bare_conf_compsoc.tex  - A bare bones starter file for IEEE Computer Society
                         conference papers.

bare_jrnl.tex          - A bare bones starter file for IEEE journal papers.

bare_jrnl_comsoc.tex   - A bare bones starter file for IEEE Communications
                         Society journal papers.

bare_jrnl_compsoc.tex  - A bare bones starter file for IEEE Computer Society
                         journal papers.

bare_jrnl_transmag.tex - A bare bones starter file for IEEE Transactions
                         on Magnetics journal papers.

bare_adv.tex           - A bare bones starter file showing advanced
                         techniques such as conditional compilation,
                         hyperlinks, PDF thumbnails, etc. The illustrated
                         format is for an IEEE Computer Society journal paper.

***************************************************************************
Legal Notice:
This code is offered as-is without any warranty either expressed or
implied; without even the implied warranty of MERCHANTABILITY or
FITNESS FOR A PARTICULAR PURPOSE! 
User assumes all risk.
In no event shall the IEEE or any contributor to this code be liable for
any damages or losses, including, but not limited to, incidental,
consequential, or any other damages, resulting from the use or misuse
of any information contained here.

All comments are the opinions of their respective authors and are not
necessarily endorsed by the IEEE.

This work is distributed under the LaTeX Project Public License (LPPL)
( http://www.latex-project.org/ ) version 1.3, and may be freely used,
distributed and modified. A copy of the LPPL, version 1.3, is included
in the base LaTeX documentation of all distributions of LaTeX released
2003/12/01 or later.
Retain all contribution notices and credits.
** Modified files should be clearly indicated as such, including  **
** renaming them and changing author support contact information. **

File list of work: IEEEtran.cls, IEEEtran_HOWTO.pdf, bare_adv.tex,
                   bare_conf.tex, bare_conf_compsoc.tex, bare_jrnl.tex,
                   bare_jrnl_comsoc.tex, bare_jrnl_compsoc.tex,
                   bare_jrnl_transmag.tex
***************************************************************************


==> IEEEtran/table_backup.tex <==
\begin{table*}[t]
% \caption{Performance (WER/CER\%) of different cross-utterance speech contexts fusion approaches on Non-Streaming C-T model evaluated on the standard dev, test sets of GigaSpeech M-size, and test set of WenetSpeech M-size pre-training datasets, where (A) stands for input audio concatenation in Section \ref{input_audio}, (B) is short for cross-utterance encoder embeddings of Section \ref{cross_encoder_emb}, (C) stands for cross-utterance encoder embedding pooling projection of Section  \ref{pooling_projection}, and (D) is chunk-based cross-utterance Encoder embeddings of Section \ref{chunk_based}. $\dagger$, $*$ denote a statistically significant (MAPSSWE\cite{gillick1989some}, $\alpha=0.05$) difference over the baseline systems (Sys.1, 13). “utt." represents utterance. “Uttlen." refers to utterance length. “Avg." means average.  “ctx." symbolizes context.}
\caption{Performance (WER/CER\%) of different cross-utterance speech contexts fusion approaches for non-streaming C-T models. The evaluation is conducted on the standard \textbf{dev} and \textbf{test} sets of the GigaSpeech M-size dataset, and the \textbf{test} set of the WenetSpeech M-size pre-training corpus. Here (A) stands for input audio concatenation in Section \ref{input_audio}, (B) is short for cross-utterance encoder embeddings of Section \ref{cross_encoder_emb}, (C) stands for cross-utterance encoder embedding pooling projection of Section  \ref{pooling_projection}, and (D) is chunk-based cross-utterance Encoder embeddings of Section \ref{chunk_based}. ``$\dagger$'' and ``$*$'' denote a statistically significant (MAPSSWE\cite{gillick1989some}, $\alpha=0.05$) difference over the baseline systems (Sys.1, 13). ``utt.'', ``Uttlen.'', ``Avg.'',   ``ctx.'' are respectively short for utterance, utterance length, average and context}.

\centering
\renewcommand\arraystretch{1.2}
\begin{tabular}{c|c|c|c|ccc|c|c|c|c|c} 
\hline\hline
\multirow{3}{*}{ID} & 
Batch&
\multirow{2}{*}{Fusion} &
\multirow{2}{*}{\#Previous utt.} &
\multicolumn{5}{c|}{GigaSpeech} &
\multicolumn{3}{c}{WenetSpeech} \\
\cline{5-12}
&mode & \multirow{2}{*}{methods} & \multirow{2}{*}{ctx. length} & \multicolumn{3}{c|}{WER} & Training & \multirow{2}{*}{RTF} & CER & Training & \multirow{2}{*}{RTF} \\
\cline{5-7}
\cline{10-10}
&training&&&DEV&TEST&Avg.& time &&TEST&time \\
\hline\hline
1 &  & - & - & 15.0 & 14.9 & 14.9& 40.1h & 0.0243 & 20.48 & 38.1h & 0.0241\\
\cline{3-12}
2 & & (A) & 1 $\times$ Uttlen. & 15.2 & 15.1 &15.1& 48.5h & 0.0257 & 20.72 & 46.3h & 0.0255\\
\cline{3-12}
3 &  &  & 1 $\times$ Uttlen. & $14.2^\dagger$ & $14.1^\dagger$ & $14.1^\dagger$ &47.2h & 0.0254 & $19.85^\dagger$ & 45.8h & 0.0250\\
4 &   & (B) & 2 $\times$ Uttlen. & $\textbf{14.1}^\dagger$ & $14.1^\dagger$ &$14.1^\dagger$ &  54.5h & 0.0257 & $19.45^\dagger$ & 52.8h & 0.0254\\
5 &   &  & 3 $\times$ Uttlen. & $\textbf{14.1}^\dagger$ & $\textbf{14.0}^\dagger$ & $\textbf{14.0}^\dagger$ &59.6h & 0.0258 & $\textbf{19.38}^\dagger$ & 57.4h & 0.0256\\
\cline{3-12}
6 &  Without&  & 1 $\times$ Uttlen. & 14.8 & 14.7 &14.7& 41.5h & 0.0251 & 20.28 & 40.0h & 0.0246\\
7 & utterance& (C) & 2 $\times$ Uttlen. & 14.6 & 14.6&14.6 & 43.7h & 0.0253 & 20.20 & 42.2h & 0.0250\\
8 &  splicing&  & 3 $\times$ Uttlen. &$14.6^\dagger$ & $14.5^\dagger$ & $14.5^\dagger$&46.2h & 0.0254 & $20.14^\dagger$ & 45.3h & 0.0245\\
\cline{3-12}
9 &  & & $\leq$60 frames & $14.6^\dagger$ & $14.6^\dagger$ & $14.6^\dagger$ &42.3h & 0.0252 & 20.23 & 41.4h & 0.0245\\
10 &   &  \multirow{2}{*}{(D)}& $\leq$100 frames & $14.5^\dagger$ & $14.5^\dagger$ & $14.5^\dagger$ &44.9h & 0.0253 & $20.04^\dagger$ & 44.1h & 0.0252\\
11 & &   & $\leq$160 frames& $14.4^\dagger$ & $14.4^\dagger$ & $14.4^\dagger$ &49.7h & 0.0256 & $19.90^\dagger$ & 48.6h & 0.0252\\
12 & & & $\leq$200 frames & $14.4^\dagger$ & $14.4^\dagger$ & $14.4^\dagger$ &53.1h & 0.0257 & $19.80^\dagger$ & 52.0h & 0.0254\\
\cline{2-12}
13  & & - & - & 15.0 & 14.9 & 14.9 &33.5h & 0.0235 & 20.45 & 32.2h & 0.0233\\
\cline{3-12}
14 &  & (A) & 1 $\times$ Uttlen. & 15.3 & 15.2 &  15.2 &41.6h & 0.0253 & 20.78 & 39.2h & 0.0251\\
\cline{3-12}
15 & &  & 1 $\times$ Uttlen. & $14.2^*$ & $14.2^*$ & $14.2^*$ &41.4h & 0.0245 & $19.82^*$ & 41.2h & 0.0244\\
16 & & (B) & 2 $\times$ Uttlen. & $\textbf{14.1}^*$ & $14.1^*$ & $14.1^*$ &48.3h & 0.0253 & $19.47^*$ & 48.1h & 0.0252\\
17 & With & & 3 $\times$ Uttlen. & $\textbf{14.1}^*$ & $\textbf{14.0}^*$ & $\textbf{14.0}^*$ & 53.4h & 0.0256 & $\textbf{19.37}^*$ & 53.1h & 0.0254\\
\cline{3-12}
18 & utterance &  & 1 $\times$ Uttlen. & 14.7 & 14.7 & 14.7 & 34.6h & 0.0236 & 20.25 & 34.3h & 0.0235\\
19 & splicing& (C) & 2 $\times$ Uttlen. & 14.6 & 14.6 & 14.6 & 36.8h & 0.0238 & $20.19^*$ & 36.5h & 0.0238\\
20 & &  & 3 $\times$ Uttlen. & $14.5^*$ & $14.5^*$ &$14.5^*$ &  40.5h & 0.0244 & $20.12^*$ & 40.3h & 0.0243\\
\cline{3-12}

21 &  & & $\leq$60 frames & $14.5^*$ & $14.5^*$ & $14.5^*$ &36.5h & 0.0238 & 20.16 & 36.6h & 0.0238\\
22 &  & \multirow{2}{*}{(D)} & $\leq$100 frames & $14.5^*$ & $14.4^*$ & $14.4^*$ &38.2h & 0.0240 & $20.02^*$ & 38.0h & 0.0241\\
23 &  &  & $\leq$160 frames & $14.4^*$ & $14.4^*$ &  $14.4^*$ & 42.6h & 0.0246 & $19.93^*$ & 42.3h & 0.0246\\
24 &  & & $\leq$200 frames & $14.4^*$ & $14.4^*$ & $14.4^*$ &47.9h & 0.0252 & $19.78^*$ & 47.6h & 0.0251\\
\hline\hline
\end{tabular}
\vspace{-2mm}
\label{exp: giga_nonstreaming}
\end{table*}


\begin{table*}[htbp]
% \caption{Performance (WER/CER\%) of cross-utterance speech contexts modelling non-streaming and streaming C-T models that are fine-tuned either: on the elderly English DEMENTIABANK PITT SPEECH dataset and Cantonese JCCOCC MoCA speech Corpus, where (A) stands for input audio concatenation in Section \ref{input_audio}, (B) in short for cross-utterance Encoder embeddings of Section \ref{cross_encoder_emb}, (C) stands for cross-utterance Encoder embeddings pooling projection of Section \ref{pooling_projection}, and (D) is chunk-based cross-utterance Encoder embeddings of Section \ref{chunk_based}. $\dagger$, $*$, $\triangle$, $\star$ denote a statistically significant (MAPSSWE\cite{gillick1989some}, $\alpha=0.05$) difference over the baseline systems (Sys.1, 6, 11, and 16). “utt." is marked as utterance, “Uttlen." is labeled as utterance length, “cur." is written as current,  “ctx." is specified as context.}
\caption{Performance (WER/CER\%) of cross-utterance speech contexts modelling approaches for non-streaming and streaming C-T models that are fine-tuned on the elderly English DEMENTIABANK PITT and Cantonese JCCOCC MoCA elderly speech datasets. ``$\dagger$'', ``$*$'', ``$\triangle$'' and ``$\star$'' denote a statistically significant (MAPSSWE\cite{gillick1989some}, $\alpha=0.05$) difference over the baseline systems (Sys.1, 6, 11, and 16). Other notations follow Table~\ref{exp: giga_nonstreaming}.}
    \centering
  \resizebox{\linewidth}{!}{
\renewcommand\arraystretch{1.2}
\begin{tabular}{c|c|c|c|c|c|c|c|cc|cc|c|c|c|c|c|c|c|c} 
\hline\hline
\multirow{4}{*}{ID} & 
\multirow{4}{*}{System} &
\multirow{2}{*}{Batch}&
 &\multirow{3}{*}{\#Previous utt.}
 &\multirow{3}{*}{\#Current utt.}
 &\multirow{1}{*}{\#Future }
 & &
\multicolumn{7}{c|}{Dementiabank Pitt WER} &
\multicolumn{5}{c}{JCCOCC MoCA CER } \\
&&\multirow{2}{*}{mode}&Fusion&\multirow{3}{*}{ctx. length} &\multirow{3}{*}{ctx. length} &\multirow{1}{*}{ ctx.}&Fine-tuned&\multicolumn{7}{c|}{(GigaSpeech $\rightarrow$ Dementiabank Pitt)}&\multicolumn{5}{c}{(WenetSpeech $\rightarrow$ JCCOCC MoCA)} \\

\cline{9-20}
& &\multirow{2}{*}{training} &method  & &&  length in&from & \multicolumn{2}{c|}{DEV} &\multicolumn{2}{c|}{EVAL} & \multirow{2}{*}{Avg.}&Fine-tuning &\multirow{2}{*}{RTF}& \multirow{2}{*}{DEV} & \multirow{2}{*}{EVAL} & \multirow{2}{*}{Avg.} & Fine-tuning &\multirow{2}{*}{RTF}\\
\cline{9-12}
& & &  & & & \multirow{1}{*}{cur. utt.}  &&    INV.& PAR. & INV. &PAR. & &time & & && &time \\
\hline\hline
1 &  &          & -   & -                  &  &  & Table \ref{exp: giga_nonstreaming}.1 & 15.41 & 35.68 & 17.59 & 25.90 &25.26 & 3.0h &0.0250& 30.10 & 27.92 & 29.01 & 8.1h & 0.0252\\
2 &  & Without  & (A) & 1 $\times$ Uttlen. & Cur. &  & Table \ref{exp: giga_nonstreaming}.2&15.80 & 36.16 & 17.94 & 26.38 & 25.70& 3.3h &0.0275& 30.28 & 28.04 & 29.16&8.9h&0.0280\\
3 &  & utterance & (B) & 3 $\times$ Uttlen. & Uttlen. & - & Table \ref{exp: giga_nonstreaming}.5 & $\textbf{15.01}$ & $\textbf{34.97}^\dagger$ & $\textbf{15.67}$ & $\textbf{25.53}$ &  $\textbf{24.70}^{\dagger}$&4.0h &0.0333& $\textbf{29.13}^{\dagger}$ & $\textbf{26.95}^{\dagger}$ & $\textbf{28.04}^{\dagger}$  & 10.1h &0.0340\\
4 &  & splicing& (C) & 3 $\times$ Uttlen. &  &  & Table \ref{exp: giga_nonstreaming}.8 & 15.30 & 35.39 & 16.08 & 25.78 & 25.03&3.3h&0.0278& 29.92 & 27.54 & 28.73&9.0h&0.0284\\
5 & Non- & & (D) & $\leq$200 frames &  &  & Table \ref{exp: giga_nonstreaming}.12 & 15.23 & 35.10 & 15.84 & 25.65 & 24.86 &3.4h&0.0283 & 29.56 & 27.13 & 28.35 & 9.2h&0.0286\\
\cline{3-20}
6 & Streaming &   &  & - &  &  & Table \ref{exp: giga_nonstreaming}.13 & 15.32 & 35.66 & 17.38 & 25.80 & 25.19 &2.6h&0.0237 & 30.12 & 27.91 & 29.02 & 7.5h&0.0241\\
7 &  & With & (A) & 1 $\times$ Uttlen. & Cur. &  & Table \ref{exp: giga_nonstreaming}.14 & 15.70 & 36.15 & 17.73 & 26.34 & 25.64&2.8h&0.0245&30.29 & 28.05 & 29.17 & 8.2h&0.0250\\
8 &  & utterance & (B) & 3 $\times$ Uttlen. & Uttlen. & - & Table \ref{exp: giga_nonstreaming}.17 & $\textbf{14.99}$ & $\textbf{34.95}^*$ & $\textbf{15.45}$ & $\textbf{25.49}$ & $\textbf{24.68}^*$& 3.4h&0.0285& $\textbf{29.12}^{*}$ & $\textbf{26.96}^*$ & $\textbf{28.04}^*$ & 9.1h&0.0291\\
9 &  & splicing & (C) & 3 $\times$ Uttlen. &  &  & Table \ref{exp: giga_nonstreaming}.20 & 15.29 & 35.38 & 15.97& 25.76 & 25.10 &2.8h &0.0247& 29.90 & 27.55 & 28.73 & 8.2h&0.0249\\

10 &  &  & (D) & $\leq$200 frames &  &  & Table \ref{exp: giga_nonstreaming}.24 &15.22 & 35.09 & 15.73 & 25.63 & 24.85&3.0h&0.0252 & 29.55 & 27.14 & 28.34 & 8.3h&0.0255\\
\hline
11 &  & & - & - & &  & Table \ref{exp: giga_streaming}.1 & 17.52 & 40.49 & 19.91 & 29.27 & 28.66&3.4h&0.0276 & 34.31 & 31.83 & 33.07 & 8.9h&0.0280\\
12 &  & Without  & (A) & 1 $\times$ Uttlen. & Cur. & \multirow{2}{*}{$\leq$20} & Table \ref{exp: giga_streaming}.2 & 17.83 & 40.92 & 20.28 & 29.47 & 29.00&3.6h&0.0310 & 34.50 & 32.13 & 33.32 & 10.0h&0.0313\\
13 &  & utterance & (B) & 3 $\times$ Uttlen. & Uttlen. & \multirow{2}{*}{frames}  & Table \ref{exp: giga_streaming}.5 & 17.12 & $39.86^{\triangle}$ & 18.24 & 28.97 & $28.14^{\triangle}$& 4.5h&0.0364& 33.72 & 31.44 & 32.58 & 11.4h&0.0373\\
14 & \multirow{2}{*}{Streaming} & splicing & (C) & 3 $\times$ Uttlen. &  &  & Table \ref{exp: giga_streaming}.8 &17.27 & 40.02 & 18.43 & 29.16 &28.30&3.6h&0.0312& 33.99 & 31.68 & 32.84 & 10.2h&0.0319\\
\cline{5-6}
15 &  & & (D) & \multicolumn{2}{c|}{$\leq$200 frames}  &  & Table \ref{exp: giga_streaming}.16 & $\textbf{16.82}^{\triangle}$ & $\textbf{39.43}^{\triangle}$ & $\textbf{17.97}$ & $\textbf{28.84}^{\triangle}$ & $\textbf{27.82}^{\triangle}$&3.8h&0.0320 & $\textbf{33.50}^{\triangle}$ & $\textbf{31.15}^{\triangle}$ & $\textbf{32.33}^{\triangle}$ & 10.4h&0.0323\\
\cline{3-20}
16 &  &  & - & - &  &  & Table \ref{exp: giga_streaming}.17 & 17.51 & 40.48 & 19.80 & 29.25 & 28.65 &3.1h& 0.0255& 34.33 & 31.84 & 33.09 & 8.1h&0.0257\\
17 &  & With & (A) & 1 $\times$ Uttlen. &Cur.  & \multirow{2}{*}{$\leq$20} & Table \ref{exp: giga_streaming}.18 & 17.82 & 40.91 & 20.17 & 29.45 & 28.99& 3.3h &0.0265& 34.51 & 32.15 & 33.33 & 9.1h&0.0270\\
18 &  & utterance  & (B) & 3 $\times$ Uttlen. & Uttlen. & \multirow{2}{*}{frames} & Table \ref{exp: giga_streaming}.21 & 17.11 & $39.85^{\star}$ & 18.13 & 28.95& $28.13^{\star}$& 4.1h&0.0325& 33.71 & 31.42 & 32.57 & 10.4h&0.0328\\
19 &  & splicing & (C) & 3 $\times$ Uttlen.&  &  & Table \ref{exp: giga_streaming}.24 & 17.26 & 40.01 & 18.32 & 29.14 & 28.29&3.3h&0.0267 & 34.01 & 31.69 & 32.85 & 9.3h&0.0271\\
\cline{5-6}
20 &  &  & (D) & \multicolumn{2}{c|}{$\leq$200 frames}  &  & Table \ref{exp: giga_streaming}.32 & $\textbf{16.81}^{\star}$ & $\textbf{39.42}^{\star}$ &$\textbf{17.86}$ & $\textbf{28.82}^{\star}$ & $\textbf{27.81}^{\star}$&3.5h &0.0285& $\textbf{33.51}^{\star}$ & $\textbf{31.15}^{\star}$ &$\textbf{32.33}^{\star}$ & 9.4h&0.0288\\

\hline\hline
\end{tabular}}
\label{exp: finetuneing_dbank_jcc}
\end{table*}


\begin{table*}[t]
% \caption{Performance (WER/CER\%) of different cross-utterance speech contexts modeling approaches on Streaming C-T model evaluated on the standard dev, test sets of GigaSpeech M-size, and test set of WenetSpeech M-size pre-training datasets, where (A) stands for input audio concatenation in Section \ref{input_audio}, (B) in short for cross-utterance Encoder embeddings of Section \ref{cross_encoder_emb}, (C) stands for cross-utterance Encoder embeddings pooling projection of Section \ref{pooling_projection}, and (D) is chunk-based cross-utterance Encoder embeddings of Section \ref{chunk_based}. $\dagger$, $*$ denote a statistically significant (MAPSSWE\cite{gillick1989some}, $\alpha=0.05$) difference over the baseline systems (Sys.1, 17). “utt." in short for utterance, “Uttlen." denotes utterance length, “cur." stands for current, “Avg." represents average,  “ctx." denotes context.}
\caption{Performance (WER/CER\%) of different cross-utterance speech contexts modeling approaches for Streaming C-T models. ``$\dagger$'' and ``$*$'' denote a statistically significant (MAPSSWE\cite{gillick1989some}, $\alpha=0.05$) difference over the baseline systems (Sys.1, 17). Other notations follow Table~\ref{exp: giga_nonstreaming}.}

\centering
% \renewcommand\arraystretch{1.2}
\setlength{\tabcolsep}{3pt} % reduce column spacing
\fontsize{8.5}{10}\selectfont % sets the font size and line 
\scalebox{0.85}{
\begin{tabular}{c|c|c|c|c|c|ccc|c|c|c|c|c} 
\hline\hline
\multirow{3}{*}{ID} & 
Batch&
\multirow{2}{*}{Fusion} &
\multirow{2}{*}{\#Previous utt.} &
\multirow{2}{*}{\#Current utt.} &
\multirow{1}{*}{\#Future ctx.} &
\multicolumn{5}{c|}{GigaSpeech} &
\multicolumn{3}{c}{WenetSpeech} \\
\cline{7-14}
&mode&\multirow{2}{*}{method}&\multirow{2}{*}{ctx. length}&\multirow{2}{*}{ctx. length}&\multirow{1}{*}{length in }&\multicolumn{3}{c|}{WER}&Training&\multirow{2}{*}{RTF}&CER&Training&\multirow{2}{*}{RTF}\\
\cline{7-9}
\cline{12-12}
 &training &  & & & cur. utt. &DEV & TEST& Avg.&time &  & TEST & time & \\
\hline\hline
1 &  & - & - & Cur. Uttlen & \multirow{16}{*}{$\leq$20 frames} & 17.7 & 17.4 &17.5& 44.9h & 0.0291 & 24.05 & 44.0h & 0.0286\\
\cline{3-5}
\cline{7-14}
2   & & (A) & 1 $\times$ Uttlen. & Cur. Uttlen &   & 17.9 & 17.6 &17.7& 52.3h & 0.0339 & 24.32 & 50.1h & 0.0325\\
\cline{3-5}
\cline{7-14}

3  &  &  & 1 $\times$ Uttlen. & &  & $17.2^\dagger$ & $17.2^\dagger$ & $17.2^\dagger$ &51.9h & 0.0337 &$23.46^\dagger$ & 49.5h & 0.0321\\
4  &  & (B) & 2 $\times$ Uttlen. & Cur. Uttlen &   & $17.0^\dagger$ & $16.9^\dagger$ & $16.9^\dagger$ & 57.3h & 0.0372 & $23.32^\dagger$ & 55.2h & 0.0358\\
5  &&  & 3 $\times$ Uttlen. & &  & $17.0^\dagger$ & $16.9^\dagger$ &$16.9^\dagger$ & 62.5h & 0.0406 & $23.30^\dagger$ & 60.4h & 0.0392\\
\cline{3-5}
\cline{7-14}
6 & Without&  & 1 $\times$ Uttlen. & &  & 17.6 & 17.5 & 17.5 &45.3h & 0.0298 & 23.80 & 44.4h & 0.0295\\
7 &utterance& (C) & 2 $\times$ Uttlen. & Cur. Uttlen &   & 17.4 & 17.4 & 17.4 &47.2h & 0.0306 & 23.65 & 46.3h & 0.0301\\
8  &splicing &  & 3 $\times$ Uttlen. & &  & $17.3^\dagger$ & $17.3^\dagger$ &  $17.3^\dagger$ &49.1h & 0.0319 & $23.50^\dagger$ & 48.2h & 0.0313\\
\cline{3-5}
\cline{7-14}
9 & & \multirow{4}{*}{-} & 0 & $\leq$60 frames&  & 17.8 & 17.5 &17.6& 44.6h & 0.0290 & 23.90 & 43.8h & 0.0284\\
10  & & & 0 & $\leq$100 frames&   & 17.7 & 17.4 &17.5& 44.8h & 0.0291 & 23.70 & 44.0h & 0.0285\\
11 & & & 0 & $\leq$160 frames&   & 17.7 & 17.4 &17.5& 45.0h & 0.0292 & 23.65 & 44.3h & 0.0288\\
12  & & & 0 & $\leq$200 frames&   & 17.7 & 17.4 &17.5& 45.0h & 0.0292 & 23.65 & 44.3h & 0.0287\\
\cline{3-5}
\cline{7-14}
13  & & & \multicolumn{2}{c|}{$\leq$60 frames}      &   & $17.1^\dagger$ & $17.0^\dagger$ & $17.0^\dagger$ & 46.7h & 0.0303 & $23.35^\dagger$ & 45.1h & 0.0296\\
14  & & \multirow{2}{*}{(D)} & \multicolumn{2}{c|}{$\leq$100 frames} &   & $17.0^\dagger$ & $16.7^\dagger$ & $16.8^\dagger$ &48.1h & 0.0312 & $23.24^\dagger$ & 46.4h & 0.0301\\
15 & &  & \multicolumn{2}{c|}{$\leq$160 frames} &   & $\textbf{16.7}^\dagger$ & $\textbf{16.4}^\dagger$ &$\textbf{16.5}^\dagger$ & 51.3h & 0.0333 & $23.10^\dagger$ & 49.5h & 0.0322\\
16  & & & \multicolumn{2}{c|}{$\leq$200 frames} &   & $\textbf{16.7}^\dagger$ & $\textbf{16.4}^\dagger$ & $\textbf{16.5}^\dagger$ &54.6h & 0.0354 & $\textbf{23.05}^\dagger$& 52.8h & 0.0343\\
\cline{2-14}
17  && - & - & Cur.Uttlen & \multirow{16}{*}{$\leq$20 frames}   & 17.7 & 17.4 & 17.5 &36.8h & 0.0254 & 24.02 & 36.1h & 0.0244\\
\cline{3-5}
\cline{7-14}
18  && (A) & 1 $\times$ Uttlen. & Cur.Uttlen &   & 17.9 & 17.7 & 17.8&44.6h & 0.0290 & 24.40 & 43.8h & 0.0284\\
\cline{3-5}
\cline{7-14}

19 & &  & 1 $\times$ Uttlen. & &   & $17.2^*$ & $17.2^*$ & $17.2^*$ &44.2h & 0.0287 & $23.44^*$ & 44.1h & 0.0286\\
20  & & (B) & 2 $\times$ Uttlen. & Cur. Uttlen &   & $17.0^*$ & $17.0^*$ & $17.0^*$ & 50.1h & 0.0325 & $23.32^*$ & 50.3h & 0.0326\\
21 &  &  & 3 $\times$ Uttlen. & &   & $17.0^*$ & $16.9^*$ & $16.9^*$ &54.3h & 0.0352 & $23.30^*$ & 54.4h & 0.0353\\
\cline{3-5}
\cline{7-14}
22  &With&  & 1 $\times$ Uttlen. & &   & 17.5 & 17.5 & 17.5 &37.2h & 0.0262 & 23.78 & 37.1h & 0.0260\\
23 &utterance& (C) & 2 $\times$ Uttlen. & Cur. Uttlen &   & 17.3 & 17.4 & 17.4&39.8h & 0.0269 & 23.66 & 39.5h & 0.0264\\
24  & splicing&& 3 $\times$ Uttlen. & &   & $17.2^*$ & 17.3 & 17.3 &42.5h & 0.0281 & 23.49 & 42.4h & 0.0276\\
\cline{3-5}
\cline{7-14}
25 & & \multirow{4}{*}{-} & 0 & $\leq$60 frames&   & 17.7 & 17.5 &  17.6 &37.2h & 0.0261 & 23.92 & 36.8h & 0.0258\\
26  & & & 0 & $\leq$100 frames&   & 17.7 & 17.4&17.5 & 37.6h & 0.0264 & 23.73 & 37.0h & 0.0260\\
27 & & & 0 & $\leq$160 frames &   & 17.7 & 17.4 &17.5& 37.9h & 0.0265 & 23.67 & 37.1h & 0.0261\\
28  & & & 0 & $\leq$200 frames &   & 17.7 & 17.4&17.5 & 37.9h & 0.0265 & 23.67 & 37.1h & 0.0262\\
\cline{3-5}
\cline{7-14}
29  & & & \multicolumn{2}{c|}{$\leq$60 frames}  &   & $17.2^*$ & $17.1^*$ & $17.1^*$ &38.0h & 0.0267 & $23.40^*$ & 37.2h & 0.0261\\
30  & & \multirow{2}{*}{(D)} & \multicolumn{2}{c|}{$\leq$100 frames} &  &$17.0^*$ & $16.8^*$ & $16.9^*$ & 40.2h & 0.0275 & $23.25^*$ & 39.6h & 0.0265\\
31  & &  & \multicolumn{2}{c|}{$\leq$160 frames}  &   & $\textbf{16.8}^*$ &$\textbf{16.4}^*$& $\textbf{16.5}^*$&43.6h & 0.0283 & $23.10^*$ & 42.8h & 0.0281\\
32  & & & \multicolumn{2}{c|}{$\leq$200 frames}  &  & $\textbf{16.8}^*$ & $\textbf{16.4}^*$& $\textbf{16.5}^*$&47.8h & 0.0310 & $\textbf{23.05}^*$ & 46.5h & 0.0304\\
\cline{4-14}
\hline\hline
\end{tabular}}

\label{exp: giga_streaming}
\end{table*}
